Don't FREAK Out: A Frequency-Inspired Approach to Detecting Backdoor Poisoned Samples in DNNs

In this paper we investigate the frequency sensitivity of Deep Neural Networks (DNNs) when presented with clean samples versus poisoned samples. Our analysis shows significant disparities in frequency sensitivity between these two types of samples. Building on these findings, we propose FREAK, a frequency-based poisoned sample detection algorithm that is simple yet effective. Our experimental results demonstrate the efficacy of FREAK not only against frequency backdoor attacks but also against some spatial attacks. Our work is just the first step in leveraging these insights. We believe that our analysis and proposed defense mechanism will provide a foundation for future research and development of backdoor defenses.

==> figures/Tables/cyo_resnet18_imagenet.tex <==
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 67.29                            & 98.57                            \\
Gaussian (3x3)   & 60.25                            & 0.00                                \\
Gaussian (5x5)   & 58.43                            & 0.00                                \\
Weiner (3x3)     & 62.11                            & 89.85                            \\
Weiner (5x5)     & 52.69                            & 88.23                            \\
Highpass         & 0.82                             & 100.00                              \\
Lowpass          & 52.71                            & 0.00                                \\
Bandpass         & 0.52                             & 92.18                            \\
JPEG Compression & 65.51                            & 57.81                            \\
Autoencoder      & 34.45                            & 0.00                                \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 65.99                            & 46.09                            \\
\quad top-$k$ = 50        & 65.61                            & 28.91                            \\
\quad top-$k$ = 125       & 65.28                            & 17.97                            \\
\rowcolor{mygray}\quad top-$k$ = 250       & 64.84                            & 10.94                            \\
\quad top-$k$ = 500       & 63.71                            & 7.81                             \\
\quad top-$k$ = 1000      & 62.41                            & 3.90                              \\ \bottomrule
\end{tabular}}

==> figures/Tables/cyo_resnet34_cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 94.33                            & 100.00                              \\
Gaussian (3x3)   & 55.43                            & 0.00                                \\
Gaussian (5x5)   & 21.80                             & 7.14                             \\
Weiner (3x3)     & 66.58                            & 7.14                             \\
Weiner (5x5)     & 46.97                            & 7.14                             \\
Highpass         & 37.91                            & 50.00                               \\
Lowpass          & 20.52                            & 7.14                             \\
Bandpass         & 28.97                            & 0.00                                \\
JPEG Compression & 87.43                            & 0.00                                \\
Autoencoder      & 83.80                             & 0.00                                \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 94.19                            & 92.85                            \\
\quad top-$k$ = 10        & 94.23                            & 78.57                            \\
\quad top-$k$ = 20        & 94.11                            & 64.29                            \\
\rowcolor{mygray}\quad top-$k$ = 50        & 93.95                            & 21.43                            \\
\quad top-$k$ = 80        & 93.58                            & 7.14                             \\
\quad top-$k$ = 100       & 93.53                            & 7.14                             \\ \bottomrule
\end{tabular}
}

==> figures/Tables/cyo_resnet34_imagenet.tex <==
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 70.63                            & 98.99                            \\
Gaussian (3x3)   & 64.12                            & 0.00                                \\
Gaussian (5x5)   & 62.57                            & 0.00                                \\
Weiner (3x3)     & 65.73                            & 22.67                            \\
Weiner (5x5)     & 57.43                            & 77.34                            \\
Highpass         & 1.10                              & 99.21                            \\
Lowpass          & 57.33                            & 0.00                                \\
Bandpass         & 0.53                             & 0.00                                \\
JPEG Compression & 69.149                           & 85.15                            \\
Autoencoder      & 38.11                            & 0.00                                \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 69.39                            & 56.25                            \\
\quad top-$k$ = 50        & 68.79                            & 47.65                            \\
\quad top-$k$ = 125       & 68.51                            & 35.94                            \\
\rowcolor{mygray}\quad top-$k$ = 250       & 68.05                            & 24.21                            \\
\quad top-$k$ = 500       & 67.23                            & 8.59                             \\
\quad top-$k$ = 1000      & 65.17                            & 1.57                             \\ \bottomrule
\end{tabular}}

==> figures/Tables/cyo_vgg19_cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 91.59                            & 100.00                              \\
Gaussian (3x3)   & 60.40                             & 0.00                                \\
Gaussian (5x5)   & 29.28                            & 7.14                             \\
Weiner (3x3)     & 62.13                            & 0.00                                \\
Weiner (5x5)     & 41.90                             & 0.00                                \\
Highpass         & 31.91                            & 50.00                               \\
Lowpass          & 25.72                            & 0.00                                \\
Bandpass         & 22.86                            & 7.14                             \\
JPEG Compression & 86.16                            & 21.43                            \\
Autoencoder      & 82.66                            & 0.00                                \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 91.63                            & 100.00                              \\
\quad top-$k$ = 10        & 91.19                            & 78.57                            \\
\quad top-$k$ = 20        & 91.11                            & 35.71                            \\
\rowcolor{mygray}\quad top-$k$ = 50        & 90.04                            & 21.42                            \\
\quad top-$k$ = 80        & 89.21                            & 7.14                             \\
\quad top-$k$ = 100       & 88.63                            & 0.00                                \\ \bottomrule
\end{tabular}
}

==> figures/Tables/cyo_vgg19_imagenet.tex <==
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 68.79                            & 100.00                              \\
Gaussian (3x3)   & 64.75                            & 98.45                            \\
Gaussian (5x5)   & 58.54                            & 3.13                            \\
Weiner (3x3)     & 64.80                             & 95.31                            \\
Weiner (5x5)     & 55.79                            & 88.28                            \\
Highpass         & 0.61                             & 100.00                              \\
Lowpass          & 54.11                            & 0.00                                \\
Bandpass         & 0.33                             & 100.00                              \\
JPEG Compression & 66.91                            & 94.53                            \\
Autoencoder      & 35.55                            & 0.00                                \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 67.95                            & 46.88                            \\
\quad top-$k$ = 50        & 67.08                            & 20.31                            \\
\quad top-$k$ = 125       & 66.08                            & 3.13                             \\
\rowcolor{mygray}\quad top-$k$ = 250       & 64.76                            & 3.91                             \\
\quad top-$k$ = 500       & 63.11                            & 3.13                             \\
\quad top-$k$ = 1000      & 59.48                            & 2.30                              \\ \bottomrule
\end{tabular}}

==> figures/Tables/defend_kl_1000.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}llrrrrr@{}}
\cmidrule(l){3-7}
                                  &              & \multicolumn{1}{l}{0.25 $\sigma$} & \multicolumn{1}{l}{0.5 $\sigma$} & \multicolumn{1}{l}{1.0 $\sigma$} & \multicolumn{1}{l}{1.5 $\sigma$} & \multicolumn{1}{l}{2.0 $\sigma$} \\ \midrule
\multirow{2}{*}{\textbf{FIBA}}    & \textbf{TPR} & 90.55                                          & 85.83                                         & 78.74                                         & 69.29                                         & 54.56                                         \\
                                  & \textbf{FPR} & 29.92                                          & 23.62                                         & 19.69                                         & 15.75                                         & 12.40                                         \\ \midrule
\multirow{2}{*}{\textbf{FTrojan}} & \textbf{TPR} & 100.00                                         & 100.00                                        & 100.00                                        & 100.00                                        & 78.74                                         \\
                                  & \textbf{FPR} & 32.28                                          & 28.35                                         & 18.90                                         & 13.39                                         & 10.54                                         \\ \midrule
\multirow{2}{*}{\textbf{CYO}}     & \textbf{TPR} & 100.00                                         & 100.00                                        & 100.00                                        & 100.00                                        & 78.74                                         \\
                                  & \textbf{FPR} & 27.56                                          & 26.77                                         & 18.11                                         & 13.39                                         & 10.54                                         \\ \bottomrule
\end{tabular}
\end{table}

==> figures/Tables/fiba_resnet18_imagenet.tex <==
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{\textbf{Method}} & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense                                & 68.51                            & 100.00                           \\
Gaussian (3x3)                            & 63.61                            & 100.00                           \\
Gaussian (5x5)                            & 59.91                            & 99.21                            \\
Weiner (3x3)                              & 64.32                            & 100.00                           \\
Weiner (5x5)                              & 55.56                            & 100.00                           \\
Highpass                                  & 1.14                             & 0.00                             \\
Lowpass                                   & 46.75                            & 100.00                           \\
Bandpass                                  & 0.72                             & 0.00                             \\
JPEG Compression                          & 66.41                            & 100.00                           \\
Autoencoder                               & 39.97                            & 71.09                            \\ \midrule
\texttt{FREAK} (ours)   & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             \\
\quad top-$k$ = 0          & \multicolumn{1}{c}{67.55}        & \multicolumn{1}{c}{96.87}        \\
\quad top-$k$ = 50         & \multicolumn{1}{c}{56.31}        & \multicolumn{1}{c}{96.87}        \\
\quad top-$k$ = 125        & \multicolumn{1}{c}{47.93}        & \multicolumn{1}{c}{96.00}        \\
\rowcolor{mygray}\quad top-$k$ = 250        & \multicolumn{1}{c}{42.01}        & \multicolumn{1}{c}{95.31}        \\
\quad top-$k$ = 500        & \multicolumn{1}{c}{37.95}        & \multicolumn{1}{c}{94.53}        \\
\quad top-$k$ = 1000       & \multicolumn{1}{c}{32.96}        & \multicolumn{1}{c}{86.81}        \\ \bottomrule
\end{tabular}}

==> figures/Tables/fiba_resnet34_cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 92.07                            & 97.52                            \\
Gaussian (3x3)   & 65.15                            & 92.85                            \\
Gaussian (5x5)   & 37.45                            & 92.85                            \\
Weiner (3x3)     & 68.98                            & 92.85                            \\
Weiner (5x5)     & 48.14                            & 92.85                            \\
Highpass         & 33.66                            & 7.41                             \\
Lowpass          & 31.27                            & 78.57                            \\
Bandpass         & 26.82                            & 14.28                            \\
JPEG Compression & 84.26                            & 92.85                            \\
Autoencoder      & 82.84                            & 85.71                            \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 92.06                            & 87.54                            \\
\quad top-$k$ = 10        & 91.32                            & 57.14                            \\
\quad top-$k$ = 20        & 89.99                            & 35.71                            \\
\rowcolor{mygray}\quad top-$k$ = 50        & 86.80                             & 7.14                             \\
\quad top-$k$ = 80        & 82.99                            & 7.14                             \\
\quad top-$k$ = 100       & 80.35                            & 7.14                             \\ \bottomrule
\end{tabular}
}

==> figures/Tables/fiba_vgg19_cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 91.14                            & 97.65                            \\
Gaussian (3x3)   & 63.00                               & 92.85                            \\
Gaussian (5x5)   & 37.43                            & 92.85                            \\
Weiner (3x3)     & 64.34                            & 92.85                            \\
Weiner (5x5)     & 45.33                            & 92.85                            \\
Highpass         & 16.28                            & 0.00                                \\
Lowpass          & 32.84                            & 92.85                            \\
Bandpass         & 13.18                            & 0.00                                \\
JPEG Compression & 85.04                            & 92.85                            \\
Autoencoder      & 82.25                            & 85.71                            \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 91.00                               & 85.71                            \\
\quad top-$k$ = 10        & 88.81                            & 57.14                            \\
\quad top-$k$ = 20        & 86.86                            & 35.71                            \\
\rowcolor{mygray}\quad top-$k$ = 50        & 81.97                            & 28.75                            \\
\quad top-$k$ = 80        & 77.57                            & 28.57                            \\
\quad top-$k$ = 100       & 74.32                            & 7.14                             \\ \bottomrule
\end{tabular}
}

==> figures/Tables/ftrojan_resnet18_imagenet.tex <==
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Method}  & \textbf{CDA}\small{(\%)} & \textbf{ASR}\small{(\%)} \\ \midrule
No Defense       & 68.25        & 100.00          \\
Gaussian (3x3)   & 62.52        & 0.00            \\
Gaussian (5x5)   & 60.09        & 0.00            \\
Weiner (3x3)     & 63.16        & 5.46         \\
Weiner (5x5)     & 55.09        & 10.90         \\
Highpass         & 1.08         & 100.00          \\
Lowpass          & 53.65        & 0.00            \\
Bandpass         & 0.58         & 0.00            \\
JPEG Compression & 66.61        & 0.00            \\
Autoencoder      & 37.95        & 0.00            \\ \midrule
\texttt {FREAK} (ours)   &              &              \\
\quad top-$k$ = 0         & 67.51        & 100.00          \\
\quad top-$k$ = 50        & 67.42        & 10.63        \\
\quad top-$k$ = 125       & 66.82        & 25.00           \\
\rowcolor{mygray}\quad top-$k$ = 250       & 66.15        & 8.61         \\
\quad top-$k$ = 500       & 64.48        & 6.25         \\
\quad top-$k$ = 1000      & 62.63        & 4.68         \\ \bottomrule
\end{tabular}}


==> figures/Tables/ftrojan_resnet34_cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 92.83                            & 100.00                              \\
Gaussian (3x3)   & 65.68                            & 0.00                                \\
Gaussian (5x5)   & 36.15                            & 14.28                            \\
Weiner (3x3)     & 68.94                            & 0.00                                \\
Weiner (5x5)     & 48.57                            & 7.14                             \\
Highpass         & 34.57                            & 100.00                              \\
Lowpass          & 29.09                            & 7.14                             \\
Bandpass         & 26.10                             & 0.00                                \\
JPEG Compression & 85.34                            & 0.00                                \\
Autoencoder      & 83.66                            & 0.00                                \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 92.66                            & 100.00                              \\
\quad top-$k$ = 10        & 92.22                            & 0.00                                \\
\quad top-$k$ = 20        & 92.18                            & 0.00                                \\
\rowcolor{mygray}\quad top-$k$ = 50        & 91.14                            & 0.00                                \\
\quad top-$k$ = 80        & 90.23                            & 0.00                                \\
\quad top-$k$ = 100       & 89.05                            & 0.00                                \\ \bottomrule
\end{tabular}
}

==> figures/Tables/ftrojan_resnet34_imagenet.tex <==
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 68.29                            & 100.00                              \\
Gaussian (3x3)   & 63.65                            & 0.00                                \\
Gaussian (5x5)   & 60.20                             & 0.00                                \\
Weiner (3x3)     & 63.43                            & 31.25                            \\
Weiner (5x5)     & 55.94                            & 15.75                            \\
Highpass         & 1.12                             & 100.00                              \\
Lowpass          & 54.77                            & 0.00                                \\
Bandpass         & 0.64                             & 0.00                                \\
JPEG Compression & 66.54                            & 0.00                                \\
Autoencoder      & 39.00                               & 0.00                                \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 67.15                            & 100.00                              \\
\quad top-$k$ = 50        & 66.98                            & 46.09                            \\
\quad top-$k$ = 125       & 66.54                            & 13.28                            \\
\rowcolor{mygray}\quad top-$k$ = 250       & 65.81                            & 9.38                             \\
\quad top-$k$ = 500       & 64.51                            & 7.03                             \\
\quad top-$k$ = 1000      & 62.43                            & 2.35                             \\ \bottomrule
\end{tabular}}

==> figures/Tables/ftrojan_vgg19_cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 91.50                             & 100.00                              \\
Gaussian (3x3)   & 61.61                            & 0.00                                \\
Gaussian (5x5)   & 36.36                            & 7.14                             \\
Weiner (3x3)     & 63.71                            & 0.00                                \\
Weiner (5x5)     & 45.85                            & 7.14                             \\
Highpass         & 19.97                            & 92.85                            \\
Lowpass          & 32.85                            & 7.14                             \\
Bandpass         & 12.31                            & 21.43                            \\
JPEG Compression & 85.87                            & 0.00                                \\
Autoencoder      & 81.90                             & 0.00                                \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 91.37                            & 100.00                              \\
\quad top-$k$ = 10        & 91.22                            & 0.00                                \\
\quad top-$k$ = 20        & 90.70                             & 0.00                                \\
\rowcolor{mygray}\quad top-$k$ = 50        & 90.02                            & 0.00                                \\
\quad top-$k$ = 80        & 88.27                            & 0.00                                \\
\quad top-$k$ = 100       & 87.09                            & 0.00                                \\ \bottomrule
\end{tabular}
}

==> figures/Tables/ftrojan_vgg19_imagenet.tex <==
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Method}  & \multicolumn{1}{c}{\textbf{CDA}\small{(\%)}} & \multicolumn{1}{c}{\textbf{ASR}\small{(\%)}} \\ \midrule
No Defense       & 68.03                            & 100.00                              \\
Gaussian (3x3)   & 63.75                            & 6.78                             \\
Gaussian (5x5)   & 59.95                            & 0.00                                \\
Weiner (3x3)     & 64.07                            & 0.00                                \\
Weiner (5x5)     & 54.06                            & 10.94                            \\
Highpass         & 0.60                              & 50.00                               \\
Lowpass          & 53.21                            & 0.00                                \\
Bandpass         & 0.35                             & 7.80                              \\
JPEG Compression & 65.62                            & 1.57                             \\
Autoencoder      & 34.87                            & 2.35                             \\ \midrule
\texttt {FREAK} (ours)   &                                  &                                  \\
\quad top-$k$ = 0         & 67.37                            & 69.54                            \\
\quad top-$k$ = 50        & 65.32                            & 3.13                             \\
\quad top-$k$ = 125       & 66.01                            & 1.57                             \\
\rowcolor{mygray}\quad top-$k$ = 250       & 65.71                            & 0.00                                \\
\quad top-$k$ = 500       & 65.48                            & 3.13                             \\
\quad top-$k$ = 1000      & 64.57                            & 0.78                             \\ \bottomrule
\end{tabular}}

==> figures/Tables/mean_and_sd.tex <==
\begin{table}[]
\begin{tabular}{lllll}
 & \multicolumn{2}{l}{Wasserstein} & \multicolumn{2}{l}{KL Divergence} \\
 &           &          &           &          \\
 &           &          &           &          \\
 &           &          &           &          \\
 &           &          &           &         
\end{tabular}
\end{table}

==> figures/Tables/resnet18_clean_cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Method}  & \textbf{CDA}\small{(\%)} \\ \midrule
No Defense       & 93.76        \\
Gaussian (3x3)   & 58.27        \\
Gaussian (5x5)   & 26.19        \\
Weiner (3x3)     & 65.38        \\
Weiner (5x5)     & 47.50         \\
Highpass         & 25.91        \\
Lowpass          & 22.33        \\
Bandpass         & 16.99        \\
JPEG Compression & 88.01        \\
Autoencoder      & 83.54        \\ \midrule
Ours             &              \\
\quad top-$k$ = 0         & 93.65        \\
\quad top-$k$ = 10        & 93.31        \\
\quad top-$k$ = 20        & 92.89        \\
\quad top-$k$ = 50        & 92.11        \\
\quad top-$k$ = 80        & 91.33        \\
\quad top-$k$ = 100       & 90.89        \\ \bottomrule
\end{tabular}
}

==> figures/Tables/resnet18_clean_imagenet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\renewcommand{\arraystretch}{1.0} 
\scalebox{0.73}{
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Method}  & \textbf{CDA}\small{(\%)} \\ \midrule
No Defense       & 66.89        \\
Gaussian (3x3)   & 62.26        \\
Gaussian (5x5)   & 58.63        \\
Weiner (3x3)     & 62.21        \\
Weiner (5x5)     & 54.11        \\
Highpass         & 0.99         \\
Lowpass          & 44.65        \\
Bandpass         & 0.57         \\
JPEG Compression & 65.48        \\
Autoencoder      & 34.42        \\ \midrule
Ours             &              \\
\quad top-$k$ = 0         & 66.08        \\
\quad top-$k$ = 50        & 64.22        \\
\quad top-$k$ = 125        & 62.39        \\
\quad top-$k$ = 250        & 60.22        \\
\quad top-$k$ = 500        & 56.55        \\
\quad top-$k$ = 1000       & 50.99        \\ \bottomrule
\end{tabular}
}
